A Response to Philippe Lemoine's Critique on our Paper "Causal Impact of Masks, Policies, Behavior on Early Covid-19 Pandemic in the U.S."

Recently, Phillippe Lemoine posted a critique of our paper "Causal Impact of Masks, Policies, Behavior on Early Covid-19 Pandemic in the U.S." [arXiv:2005.14168] at his post titled "Lockdowns, econometrics and the art of putting lipstick on a pig." Although Lemoine's critique appears ideologically driven and overly emotional, some of his points are worth addressing. In particular, the sensitivity of our estimation results for (i) including "masks in public spaces" and (ii) updating the data seems important critiques and, therefore, we decided to analyze the updated data ourselves. This note summarizes our findings from re-examining the updated data and responds to Phillippe Lemoine's critique on these two important points. We also briefly discuss other points Lemoine raised in his post. After analyzing the updated data, we find evidence that reinforces the conclusions reached in the original study.

==> tables_and_figures/casecor.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:35:59 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:38 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & NYT & JHU & CTP \\ 
  \hline
NYT & 1.00000 & 0.99985 & 0.99970 \\ 
  JHU & 0.99985 & 1.00000 & 0.99985 \\ 
  CTP & 0.99970 & 0.99985 & 1.00000 \\ 
   \hline
\end{tabular}
\caption{Correlation of cumulative cases \label{tab:casecor}} 
\end{table}


==> tables_and_figures/casediff.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:35:59 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:38 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & 1 & 2 & 3 \\ 
  \hline
NYT & 1.00 & 0.38 & 0.32 \\ 
  JHU & 0.38 & 1.00 & 0.51 \\ 
  CTP & 0.32 & 0.51 & 1.00 \\ 
   \hline
\end{tabular}
\caption{Portion of cumulative cases that are equal between data sets\label{tab:casediff}} 
\end{table}


==> tables_and_figures/cases-maskall-long-dec-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employeesonly, 14) & $-$0.052$^{***}$ & $-$0.052$^{***}$ & $-$0.048$^{***}$ & $-$0.047$^{***}$ \\ 
  & (0.017) & (0.018) & (0.014) & (0.015) \\ 
  lag(masks in public spaces, 14) & $-$0.072$^{***}$ & $-$0.071$^{***}$ & $-$0.067$^{***}$ & $-$0.064$^{***}$ \\ 
  & (0.021) & (0.022) & (0.018) & (0.019) \\ 
  lag(closed K-12 schools, 14) & $-$0.149$^{***}$ & $-$0.152$^{***}$ & $-$0.077$^{***}$ & $-$0.080$^{***}$ \\ 
  & (0.039) & (0.040) & (0.029) & (0.030) \\ 
  lag(stay at home, 14) & $-$0.052$^{*}$ & $-$0.054$^{*}$ & $-$0.041 & $-$0.044 \\ 
  & (0.031) & (0.031) & (0.031) & (0.031) \\ 
  lag(business closure policies, 14) & $-$0.133$^{***}$ &  & $-$0.085$^{**}$ &  \\ 
  & (0.037) &  & (0.039) &  \\ 
  lag(closed movie theaters, 14) &  & $-$0.069$^{***}$ &  & $-$0.058$^{***}$ \\ 
  &  & (0.019) &  & (0.019) \\ 
  lag(closed restaurants, 14) &  & $-$0.001 &  & 0.009 \\ 
  &  & (0.047) &  & (0.049) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.046 &  & $-$0.010 \\ 
  &  & (0.039) &  & (0.039) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.073$^{***}$ & 0.073$^{***}$ & 0.060$^{***}$ & 0.061$^{***}$ \\ 
  & (0.014) & (0.014) & (0.016) & (0.016) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.118$^{***}$ & $-$0.119$^{***}$ & $-$0.091$^{***}$ & $-$0.093$^{***}$ \\ 
  & (0.009) & (0.010) & (0.009) & (0.009) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.051 & $-$0.052 \\ 
  &  &  & (0.039) & (0.040) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.154$^{***}$ & $-$0.156$^{***}$ \\ 
  &  &  & (0.018) & (0.019) \\ 
  $\Delta \log T_{it}$ & 0.117$^{***}$ & 0.117$^{***}$ & 0.114$^{***}$ & 0.113$^{***}$ \\ 
  & (0.030) & (0.030) & (0.029) & (0.029) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.459$^{***}$ & -0.444$^{***}$ & -0.318$^{***}$ & -0.295$^{***}$ \\ 
 & (0.066) & (0.069) & (0.063) & (0.068) \\ 
Observations & 13,461 & 13,461 & 13,461 & 13,461 \\ 
R$^{2}$ & 0.429 & 0.429 & 0.435 & 0.436 \\ 
Adjusted R$^{2}$ & 0.426 & 0.426 & 0.432 & 0.432 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-long-oct-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.058$^{***}$ & $-$0.058$^{***}$ & $-$0.057$^{***}$ & $-$0.056$^{***}$ \\ 
  & (0.019) & (0.020) & (0.017) & (0.018) \\ 
  lag(masks in public spaces, 14) & $-$0.111$^{***}$ & $-$0.107$^{***}$ & $-$0.108$^{***}$ & $-$0.102$^{***}$ \\ 
  & (0.026) & (0.028) & (0.024) & (0.026) \\ 
  lag(closed K-12 schools, 14) & $-$0.140$^{***}$ & $-$0.143$^{***}$ & $-$0.059 & $-$0.061 \\ 
  & (0.047) & (0.048) & (0.036) & (0.037) \\ 
  lag(stay at home, 14) & $-$0.068$^{**}$ & $-$0.071$^{**}$ & $-$0.056 & $-$0.062$^{*}$ \\ 
  & (0.033) & (0.034) & (0.034) & (0.035) \\ 
  lag(business closure policies, 14) & $-$0.121$^{***}$ &  & $-$0.076$^{*}$ &  \\ 
  & (0.041) &  & (0.042) &  \\ 
  lag(closed movie theaters, 14) &  & $-$0.074$^{***}$ &  & $-$0.066$^{***}$ \\ 
  &  & (0.023) &  & (0.023) \\ 
  lag(closed restaurants, 14) &  & 0.010 &  & 0.021 \\ 
  &  & (0.048) &  & (0.050) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.039 &  & $-$0.007 \\ 
  &  & (0.039) &  & (0.039) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.073$^{***}$ & 0.073$^{***}$ & 0.059$^{***}$ & 0.060$^{***}$ \\ 
  & (0.013) & (0.013) & (0.015) & (0.015) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.120$^{***}$ & $-$0.121$^{***}$ & $-$0.094$^{***}$ & $-$0.096$^{***}$ \\ 
  & (0.010) & (0.010) & (0.010) & (0.011) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.052 & $-$0.056 \\ 
  &  &  & (0.042) & (0.044) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.153$^{***}$ & $-$0.156$^{***}$ \\ 
  &  &  & (0.023) & (0.023) \\ 
  $\Delta \log T_{it}$ & 0.129$^{***}$ & 0.129$^{***}$ & 0.126$^{***}$ & 0.125$^{***}$ \\ 
  & (0.036) & (0.036) & (0.034) & (0.034) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.497$^{***}$ & -0.483$^{***}$ & -0.356$^{***}$ & -0.334$^{***}$ \\ 
 & (0.078) & (0.081) & (0.074) & (0.080) \\ 
Observations & 9,842 & 9,842 & 9,842 & 9,842 \\ 
R$^{2}$ & 0.443 & 0.444 & 0.449 & 0.449 \\ 
Adjusted R$^{2}$ & 0.440 & 0.440 & 0.445 & 0.445 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-long-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employeesonly, 14) & $-$0.051$^{***}$ & $-$0.051$^{***}$ & $-$0.047$^{***}$ & $-$0.046$^{***}$ \\ 
  & (0.017) & (0.018) & (0.014) & (0.015) \\ 
  lag(masks in public spaces, 14) & $-$0.072$^{***}$ & $-$0.070$^{***}$ & $-$0.067$^{***}$ & $-$0.063$^{***}$ \\ 
  & (0.021) & (0.022) & (0.018) & (0.019) \\ 
  lag(closed K-12 schools, 14) & $-$0.149$^{***}$ & $-$0.152$^{***}$ & $-$0.078$^{***}$ & $-$0.081$^{***}$ \\ 
  & (0.039) & (0.040) & (0.029) & (0.030) \\ 
  lag(stay at home, 14) & $-$0.052$^{*}$ & $-$0.054$^{*}$ & $-$0.041 & $-$0.044 \\ 
  & (0.031) & (0.031) & (0.031) & (0.031) \\ 
  lag(business closure policies, 14) & $-$0.133$^{***}$ &  & $-$0.085$^{**}$ &  \\ 
  & (0.037) &  & (0.039) &  \\ 
  lag(closed movie theaters, 14) &  & $-$0.068$^{***}$ &  & $-$0.058$^{***}$ \\ 
  &  & (0.019) &  & (0.019) \\ 
  lag(closed restaurants, 14) &  & $-$0.001 &  & 0.009 \\ 
  &  & (0.047) &  & (0.049) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.046 &  & $-$0.010 \\ 
  &  & (0.039) &  & (0.039) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.073$^{***}$ & 0.073$^{***}$ & 0.060$^{***}$ & 0.061$^{***}$ \\ 
  & (0.014) & (0.014) & (0.016) & (0.016) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.118$^{***}$ & $-$0.119$^{***}$ & $-$0.091$^{***}$ & $-$0.093$^{***}$ \\ 
  & (0.009) & (0.010) & (0.009) & (0.009) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.051 & $-$0.052 \\ 
  &  &  & (0.039) & (0.040) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.154$^{***}$ & $-$0.156$^{***}$ \\ 
  &  &  & (0.018) & (0.019) \\ 
  $\Delta \log T_{it}$ & 0.117$^{***}$ & 0.117$^{***}$ & 0.114$^{***}$ & 0.113$^{***}$ \\ 
  & (0.030) & (0.030) & (0.029) & (0.029) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.457$^{***}$ & -0.442$^{***}$ & -0.317$^{***}$ & -0.294$^{***}$ \\ 
 & (0.066) & (0.069) & (0.063) & (0.069) \\ 
Observations & 13,461 & 13,461 & 13,461 & 13,461 \\ 
R$^{2}$ & 0.429 & 0.429 & 0.435 & 0.436 \\ 
Adjusted R$^{2}$ & 0.426 & 0.426 & 0.432 & 0.432 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-nohawaii-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.056 & $-$0.056 & $-$0.078$^{**}$ & $-$0.079$^{**}$ \\ 
  & (0.043) & (0.043) & (0.036) & (0.037) \\ 
  lag(masks in public spaces, 14) & $-$0.061 & $-$0.051 & $-$0.099$^{**}$ & $-$0.090$^{*}$ \\ 
  & (0.039) & (0.044) & (0.042) & (0.046) \\ 
  lag(closed K-12 schools, 14) & $-$0.164$^{**}$ & $-$0.164$^{*}$ & 0.050 & 0.046 \\ 
  & (0.083) & (0.089) & (0.105) & (0.109) \\ 
  lag(stay at home, 14) & $-$0.114$^{*}$ & $-$0.115$^{*}$ & $-$0.115$^{**}$ & $-$0.109$^{*}$ \\ 
  & (0.061) & (0.059) & (0.058) & (0.056) \\ 
  lag(business closure policies, 14) & $-$0.056 &  & 0.006 &  \\ 
  & (0.071) &  & (0.065) &  \\ 
  lag(closed movie theaters, 14) &  & 0.027 &  & 0.049 \\ 
  &  & (0.055) &  & (0.051) \\ 
  lag(closed restaurants, 14) &  & $-$0.053 &  & $-$0.019 \\ 
  &  & (0.048) &  & (0.045) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.020 &  & $-$0.013 \\ 
  &  & (0.050) &  & (0.044) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.039 & 0.042$^{*}$ & 0.045 & 0.045 \\ 
  & (0.024) & (0.024) & (0.027) & (0.027) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.164$^{***}$ & $-$0.166$^{***}$ & $-$0.123$^{***}$ & $-$0.123$^{***}$ \\ 
  & (0.017) & (0.018) & (0.016) & (0.016) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.140$^{***}$ & $-$0.135$^{***}$ \\ 
  &  &  & (0.038) & (0.041) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.219$^{***}$ & $-$0.219$^{***}$ \\ 
  &  &  & (0.036) & (0.036) \\ 
  $\Delta \log T_{it}$ & 0.110$^{***}$ & 0.111$^{***}$ & 0.113$^{***}$ & 0.113$^{***}$ \\ 
  & (0.028) & (0.028) & (0.027) & (0.026) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.450$^{***}$ & -0.432$^{***}$ & -0.235 & -0.215 \\ 
 & (0.157) & (0.164) & (0.177) & (0.185) \\ 
Observations & 3,735 & 3,735 & 3,735 & 3,735 \\ 
R$^{2}$ & 0.769 & 0.769 & 0.779 & 0.779 \\ 
Adjusted R$^{2}$ & 0.767 & 0.767 & 0.777 & 0.777 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-revised-noCT-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.146$^{***}$ & $-$0.146$^{***}$ & $-$0.147$^{***}$ & $-$0.151$^{***}$ \\ 
  & (0.044) & (0.045) & (0.034) & (0.033) \\ 
  lag(masks in public spaces, 14) & $-$0.069$^{*}$ & $-$0.068 & $-$0.109$^{***}$ & $-$0.112$^{***}$ \\ 
  & (0.042) & (0.043) & (0.042) & (0.042) \\ 
  lag(closed K-12 schools, 14) & $-$0.202$^{***}$ & $-$0.202$^{***}$ & $-$0.064 & $-$0.066 \\ 
  & (0.065) & (0.066) & (0.070) & (0.069) \\ 
  lag(stay at home, 14) & $-$0.100$^{*}$ & $-$0.101$^{*}$ & $-$0.103$^{*}$ & $-$0.099$^{*}$ \\ 
  & (0.057) & (0.060) & (0.056) & (0.059) \\ 
  lag(business closure policies, 14) & $-$0.053 &  & 0.019 &  \\ 
  & (0.053) &  & (0.052) &  \\ 
  lag(closed movie theaters, 14) &  & 0.001 &  & 0.016 \\ 
  &  & (0.060) &  & (0.064) \\ 
  lag(closed restaurants, 14) &  & $-$0.040 &  & 0.015 \\ 
  &  & (0.053) &  & (0.057) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.012 &  & $-$0.011 \\ 
  &  & (0.041) &  & (0.033) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.061$^{**}$ & 0.062$^{**}$ & 0.052$^{*}$ & 0.051$^{*}$ \\ 
  & (0.024) & (0.025) & (0.027) & (0.027) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.133$^{***}$ & $-$0.134$^{***}$ & $-$0.090$^{***}$ & $-$0.089$^{***}$ \\ 
  & (0.019) & (0.020) & (0.024) & (0.024) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.119$^{***}$ & $-$0.121$^{***}$ \\ 
  &  &  & (0.041) & (0.046) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.216$^{***}$ & $-$0.217$^{***}$ \\ 
  &  &  & (0.040) & (0.040) \\ 
  $\Delta \log T_{it}$ & 0.167$^{***}$ & 0.167$^{***}$ & 0.163$^{***}$ & 0.163$^{***}$ \\ 
  & (0.046) & (0.046) & (0.043) & (0.043) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.569$^{***}$ & -0.566$^{***}$ & -0.404$^{***}$ & -0.409$^{***}$ \\ 
 & (0.135) & (0.137) & (0.131) & (0.134) \\ 
Observations & 3,651 & 3,651 & 3,651 & 3,651 \\ 
R$^{2}$ & 0.737 & 0.737 & 0.749 & 0.749 \\ 
Adjusted R$^{2}$ & 0.735 & 0.735 & 0.747 & 0.746 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-revised-noMT-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.142$^{***}$ & $-$0.147$^{***}$ & $-$0.141$^{***}$ & $-$0.148$^{***}$ \\ 
  & (0.043) & (0.043) & (0.031) & (0.030) \\ 
  lag(masks in public spaces, 14) & $-$0.059 & $-$0.058 & $-$0.101$^{**}$ & $-$0.105$^{***}$ \\ 
  & (0.040) & (0.041) & (0.040) & (0.041) \\ 
  lag(closed K-12 schools, 14) & $-$0.190$^{***}$ & $-$0.192$^{***}$ & $-$0.054 & $-$0.057 \\ 
  & (0.067) & (0.067) & (0.072) & (0.071) \\ 
  lag(stay at home, 14) & $-$0.076$^{*}$ & $-$0.074 & $-$0.070$^{*}$ & $-$0.064 \\ 
  & (0.045) & (0.046) & (0.042) & (0.044) \\ 
  lag(business closure policies, 14) & $-$0.047 &  & 0.023 &  \\ 
  & (0.046) &  & (0.045) &  \\ 
  lag(closed movie theaters, 14) &  & 0.040 &  & 0.050 \\ 
  &  & (0.055) &  & (0.058) \\ 
  lag(closed restaurants, 14) &  & $-$0.060 &  & $-$0.004 \\ 
  &  & (0.052) &  & (0.056) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.022 &  & $-$0.018 \\ 
  &  & (0.038) &  & (0.031) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.057$^{**}$ & 0.059$^{**}$ & 0.045$^{*}$ & 0.045$^{*}$ \\ 
  & (0.024) & (0.025) & (0.026) & (0.026) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.141$^{***}$ & $-$0.142$^{***}$ & $-$0.093$^{***}$ & $-$0.092$^{***}$ \\ 
  & (0.021) & (0.022) & (0.028) & (0.028) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.102$^{**}$ & $-$0.101$^{**}$ \\ 
  &  &  & (0.040) & (0.043) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.214$^{***}$ & $-$0.215$^{***}$ \\ 
  &  &  & (0.042) & (0.042) \\ 
  $\Delta \log T_{it}$ & 0.172$^{***}$ & 0.172$^{***}$ & 0.169$^{***}$ & 0.169$^{***}$ \\ 
  & (0.047) & (0.047) & (0.043) & (0.043) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.514$^{***}$ & -0.512$^{***}$ & -0.342$^{***}$ & -0.346$^{***}$ \\ 
 & (0.135) & (0.139) & (0.126) & (0.129) \\ 
Observations & 3,651 & 3,651 & 3,651 & 3,651 \\ 
R$^{2}$ & 0.756 & 0.756 & 0.768 & 0.768 \\ 
Adjusted R$^{2}$ & 0.754 & 0.754 & 0.765 & 0.765 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-revised-noND-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.140$^{***}$ & $-$0.143$^{***}$ & $-$0.141$^{***}$ & $-$0.148$^{***}$ \\ 
  & (0.044) & (0.045) & (0.032) & (0.032) \\ 
  lag(masks in public spaces, 14) & $-$0.069$^{*}$ & $-$0.070$^{*}$ & $-$0.108$^{***}$ & $-$0.113$^{***}$ \\ 
  & (0.042) & (0.042) & (0.040) & (0.041) \\ 
  lag(closed K-12 schools, 14) & $-$0.205$^{***}$ & $-$0.207$^{***}$ & $-$0.069 & $-$0.072 \\ 
  & (0.067) & (0.068) & (0.072) & (0.072) \\ 
  lag(stay at home, 14) & $-$0.084$^{*}$ & $-$0.082$^{*}$ & $-$0.081$^{*}$ & $-$0.077$^{*}$ \\ 
  & (0.047) & (0.048) & (0.045) & (0.046) \\ 
  lag(business closure policies, 14) & $-$0.070 &  & 0.002 &  \\ 
  & (0.056) &  & (0.053) &  \\ 
  lag(closed movie theaters, 14) &  & 0.003 &  & 0.020 \\ 
  &  & (0.061) &  & (0.065) \\ 
  lag(closed restaurants, 14) &  & $-$0.040 &  & 0.010 \\ 
  &  & (0.056) &  & (0.060) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.030 &  & $-$0.026 \\ 
  &  & (0.041) &  & (0.034) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.064$^{***}$ & 0.065$^{***}$ & 0.056$^{**}$ & 0.056$^{**}$ \\ 
  & (0.024) & (0.025) & (0.027) & (0.027) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.136$^{***}$ & $-$0.136$^{***}$ & $-$0.092$^{***}$ & $-$0.091$^{***}$ \\ 
  & (0.019) & (0.020) & (0.025) & (0.025) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.111$^{***}$ & $-$0.113$^{**}$ \\ 
  &  &  & (0.041) & (0.046) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.211$^{***}$ & $-$0.212$^{***}$ \\ 
  &  &  & (0.040) & (0.040) \\ 
  $\Delta \log T_{it}$ & 0.163$^{***}$ & 0.163$^{***}$ & 0.160$^{***}$ & 0.160$^{***}$ \\ 
  & (0.046) & (0.046) & (0.043) & (0.043) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.568$^{***}$ & -0.569$^{***}$ & -0.397$^{***}$ & -0.406$^{***}$ \\ 
 & (0.139) & (0.143) & (0.136) & (0.141) \\ 
Observations & 3,654 & 3,654 & 3,654 & 3,654 \\ 
R$^{2}$ & 0.748 & 0.748 & 0.759 & 0.759 \\ 
Adjusted R$^{2}$ & 0.745 & 0.745 & 0.756 & 0.756 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-revised-noVT-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.125$^{***}$ & $-$0.127$^{***}$ & $-$0.132$^{***}$ & $-$0.137$^{***}$ \\ 
  & (0.048) & (0.048) & (0.035) & (0.034) \\ 
  lag(masks in public spaces, 14) & $-$0.063 & $-$0.063 & $-$0.106$^{***}$ & $-$0.109$^{***}$ \\ 
  & (0.040) & (0.040) & (0.040) & (0.040) \\ 
  lag(closed K-12 schools, 14) & $-$0.195$^{***}$ & $-$0.197$^{***}$ & $-$0.058 & $-$0.061 \\ 
  & (0.068) & (0.068) & (0.068) & (0.066) \\ 
  lag(stay at home, 14) & $-$0.071 & $-$0.069 & $-$0.068 & $-$0.063 \\ 
  & (0.048) & (0.050) & (0.045) & (0.047) \\ 
  lag(business closure policies, 14) & $-$0.050 &  & 0.021 &  \\ 
  & (0.049) &  & (0.048) &  \\ 
  lag(closed movie theaters, 14) &  & 0.021 &  & 0.037 \\ 
  &  & (0.058) &  & (0.061) \\ 
  lag(closed restaurants, 14) &  & $-$0.049 &  & 0.003 \\ 
  &  & (0.051) &  & (0.055) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.019 &  & $-$0.016 \\ 
  &  & (0.038) &  & (0.032) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.066$^{***}$ & 0.068$^{***}$ & 0.055$^{**}$ & 0.055$^{**}$ \\ 
  & (0.024) & (0.024) & (0.027) & (0.027) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.136$^{***}$ & $-$0.137$^{***}$ & $-$0.091$^{***}$ & $-$0.090$^{***}$ \\ 
  & (0.021) & (0.022) & (0.026) & (0.026) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.112$^{***}$ & $-$0.112$^{**}$ \\ 
  &  &  & (0.041) & (0.045) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.216$^{***}$ & $-$0.217$^{***}$ \\ 
  &  &  & (0.040) & (0.040) \\ 
  $\Delta \log T_{it}$ & 0.163$^{***}$ & 0.163$^{***}$ & 0.159$^{***}$ & 0.160$^{***}$ \\ 
  & (0.046) & (0.045) & (0.042) & (0.042) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.504$^{***}$ & -0.502$^{***}$ & -0.344$^{***}$ & -0.346$^{**}$ \\ 
 & (0.147) & (0.149) & (0.133) & (0.135) \\ 
Observations & 3,651 & 3,651 & 3,651 & 3,651 \\ 
R$^{2}$ & 0.744 & 0.744 & 0.756 & 0.756 \\ 
Adjusted R$^{2}$ & 0.742 & 0.742 & 0.753 & 0.753 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/cases-maskall-revised-noWV-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta C_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 14) & $-$0.139$^{***}$ & $-$0.138$^{***}$ & $-$0.142$^{***}$ & $-$0.146$^{***}$ \\ 
  & (0.042) & (0.042) & (0.031) & (0.030) \\ 
  lag(masks in public spaces, 14) & $-$0.073$^{*}$ & $-$0.071$^{*}$ & $-$0.114$^{***}$ & $-$0.118$^{***}$ \\ 
  & (0.042) & (0.042) & (0.041) & (0.041) \\ 
  lag(closed K-12 schools, 14) & $-$0.203$^{***}$ & $-$0.203$^{***}$ & $-$0.067 & $-$0.069 \\ 
  & (0.069) & (0.070) & (0.073) & (0.072) \\ 
  lag(stay at home, 14) & $-$0.091$^{*}$ & $-$0.092$^{*}$ & $-$0.089$^{*}$ & $-$0.086$^{*}$ \\ 
  & (0.050) & (0.050) & (0.048) & (0.049) \\ 
  lag(business closure policies, 14) & $-$0.047 &  & 0.025 &  \\ 
  & (0.053) &  & (0.052) &  \\ 
  lag(closed movie theaters, 14) &  & $-$0.004 &  & 0.011 \\ 
  &  & (0.059) &  & (0.062) \\ 
  lag(closed restaurants, 14) &  & $-$0.031 &  & 0.026 \\ 
  &  & (0.055) &  & (0.056) \\ 
  lag(closed non-essent bus, 14) &  & $-$0.011 &  & $-$0.012 \\ 
  &  & (0.038) &  & (0.031) \\ 
  lag($\Delta \log \Delta C_{it}$, 14) & 0.063$^{**}$ & 0.064$^{**}$ & 0.055$^{**}$ & 0.055$^{**}$ \\ 
  & (0.025) & (0.025) & (0.027) & (0.027) \\ 
  lag($\log \Delta C_{it}$, 14) & $-$0.136$^{***}$ & $-$0.136$^{***}$ & $-$0.091$^{***}$ & $-$0.091$^{***}$ \\ 
  & (0.020) & (0.020) & (0.025) & (0.026) \\ 
  lag($\Delta \log \Delta C_{it}$.national, 14) &  &  & $-$0.120$^{***}$ & $-$0.124$^{***}$ \\ 
  &  &  & (0.040) & (0.044) \\ 
  lag($\log \Delta C_{it}$.national, 14) &  &  & $-$0.218$^{***}$ & $-$0.220$^{***}$ \\ 
  &  &  & (0.040) & (0.040) \\ 
  $\Delta \log T_{it}$ & 0.175$^{***}$ & 0.175$^{***}$ & 0.171$^{***}$ & 0.171$^{***}$ \\ 
  & (0.047) & (0.047) & (0.044) & (0.044) \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.552$^{***}$ & -0.550$^{***}$ & -0.387$^{***}$ & -0.393$^{***}$ \\ 
 & (0.138) & (0.141) & (0.135) & (0.138) \\ 
Observations & 3,657 & 3,657 & 3,657 & 3,657 \\ 
R$^{2}$ & 0.743 & 0.743 & 0.755 & 0.755 \\ 
Adjusted R$^{2}$ & 0.741 & 0.741 & 0.753 & 0.753 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-maskall-long-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employeesonly, 21) & $-$0.031 & $-$0.024 & $-$0.040$^{**}$ & $-$0.032 \\ 
  & (0.023) & (0.024) & (0.019) & (0.021) \\ 
  lag(masks in public spaces, 21) & $-$0.043$^{*}$ & $-$0.034 & $-$0.051$^{***}$ & $-$0.039$^{*}$ \\ 
  & (0.022) & (0.024) & (0.019) & (0.020) \\ 
  lag(closed K-12 schools, 21) & $-$0.343$^{***}$ & $-$0.338$^{***}$ & $-$0.153$^{***}$ & $-$0.146$^{***}$ \\ 
  & (0.115) & (0.113) & (0.057) & (0.050) \\ 
  lag(stay at home, 21) & $-$0.015 & $-$0.024 & $-$0.010 & $-$0.020 \\ 
  & (0.034) & (0.034) & (0.033) & (0.032) \\ 
  lag(business closure policies, 21) & $-$0.169$^{***}$ &  & $-$0.039 &  \\ 
  & (0.065) &  & (0.054) &  \\ 
  lag(closed movie theaters, 21) &  & $-$0.070$^{**}$ &  & $-$0.046$^{*}$ \\ 
  &  & (0.028) &  & (0.026) \\ 
  lag(closed restaurants, 21) &  & $-$0.133$^{**}$ &  & $-$0.066 \\ 
  &  & (0.058) &  & (0.048) \\ 
  lag(closed non-essent bus, 21) &  & 0.066 &  & 0.129$^{***}$ \\ 
  &  & (0.048) &  & (0.049) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & 0.031 & 0.035 & 0.034 & 0.036 \\ 
  & (0.032) & (0.032) & (0.035) & (0.035) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.097$^{***}$ & $-$0.101$^{***}$ & $-$0.074$^{***}$ & $-$0.078$^{***}$ \\ 
  & (0.011) & (0.011) & (0.007) & (0.007) \\ 
  lag($\Delta \log \Delta D_{it}$.national, 21) &  &  & $-$0.077 & $-$0.066 \\ 
  &  &  & (0.055) & (0.056) \\ 
  lag($\log \Delta D_{it}$.national, 21) &  &  & $-$0.114$^{***}$ & $-$0.120$^{***}$ \\ 
  &  &  & (0.020) & (0.020) \\ 
   &  &  &  &  \\ 
  &  &  &  &  \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.600$^{***}$ & -0.557$^{***}$ & -0.293$^{***}$ & -0.220$^{**}$ \\ 
 & (0.102) & (0.105) & (0.091) & (0.096) \\ 
Observations & 13,209 & 13,209 & 13,209 & 13,209 \\ 
R$^{2}$ & 0.232 & 0.233 & 0.238 & 0.240 \\ 
Adjusted R$^{2}$ & 0.227 & 0.228 & 0.234 & 0.235 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-maskall-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 21) & $-$0.159$^{***}$ & $-$0.160$^{***}$ & $-$0.181$^{***}$ & $-$0.183$^{***}$ \\ 
  & (0.059) & (0.061) & (0.059) & (0.062) \\ 
  lag(masks in public spaces, 21) & $-$0.110$^{*}$ & $-$0.107 & $-$0.133$^{**}$ & $-$0.126$^{*}$ \\ 
  & (0.065) & (0.069) & (0.064) & (0.066) \\ 
  lag(closed K-12 schools, 21) & $-$0.611$^{***}$ & $-$0.622$^{***}$ & $-$0.234$^{**}$ & $-$0.249$^{**}$ \\ 
  & (0.115) & (0.120) & (0.111) & (0.109) \\ 
  lag(stay at home, 21) & $-$0.081 & $-$0.074 & $-$0.067 & $-$0.055 \\ 
  & (0.067) & (0.065) & (0.067) & (0.062) \\ 
  lag(business closure policies, 21) & $-$0.061 &  & 0.057 &  \\ 
  & (0.087) &  & (0.086) &  \\ 
  lag(closed movie theaters, 21) &  & $-$0.003 &  & 0.054 \\ 
  &  & (0.090) &  & (0.084) \\ 
  lag(closed restaurants, 21) &  & $-$0.014 &  & 0.028 \\ 
  &  & (0.062) &  & (0.055) \\ 
  lag(closed non-essent bus, 21) &  & $-$0.043 &  & $-$0.019 \\ 
  &  & (0.068) &  & (0.064) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & $-$0.0005 & $-$0.001 & 0.017 & 0.016 \\ 
  & (0.033) & (0.033) & (0.036) & (0.036) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.078$^{***}$ & $-$0.077$^{***}$ & $-$0.063$^{**}$ & $-$0.062$^{**}$ \\ 
  & (0.026) & (0.027) & (0.027) & (0.028) \\ 
  lag($\Delta \log \Delta D_{it}$.national, 21) &  &  & $-$0.147$^{***}$ & $-$0.148$^{**}$ \\ 
  &  &  & (0.056) & (0.057) \\ 
  lag($\log \Delta D_{it}$.national, 21) &  &  & $-$0.116$^{***}$ & $-$0.117$^{***}$ \\ 
  &  &  & (0.032) & (0.032) \\ 
   &  &  &  &  \\ 
  &  &  &  &  \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -1.022$^{***}$ & -1.023$^{***}$ & -0.558$^{***}$ & -0.551$^{**}$ \\ 
 & (0.199) & (0.209) & (0.216) & (0.224) \\ 
Observations & 3,468 & 3,468 & 3,468 & 3,468 \\ 
R$^{2}$ & 0.502 & 0.502 & 0.512 & 0.512 \\ 
Adjusted R$^{2}$ & 0.497 & 0.497 & 0.507 & 0.507 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/deaths-maskall-revised-piy.tex <==
\begin{tabular}{@{\extracolsep{1pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
 & \multicolumn{4}{c}{$\Delta \log \Delta D_{it}$} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 lag(masks for employees only, 21) & $-$0.099$^{*}$ & $-$0.081 & $-$0.113$^{**}$ & $-$0.101$^{*}$ \\ 
  & (0.053) & (0.057) & (0.053) & (0.058) \\ 
  lag(masks in public spaces, 21) & $-$0.034 & $-$0.016 & $-$0.065 & $-$0.053 \\ 
  & (0.084) & (0.092) & (0.082) & (0.088) \\ 
  lag(closed K-12 schools, 21) & $-$0.513$^{***}$ & $-$0.483$^{***}$ & $-$0.210$^{***}$ & $-$0.196$^{***}$ \\ 
  & (0.105) & (0.109) & (0.075) & (0.075) \\ 
  lag(stay at home, 21) & $-$0.057 & $-$0.074 & $-$0.051 & $-$0.060 \\ 
  & (0.061) & (0.060) & (0.059) & (0.057) \\ 
  lag(business closure policies, 21) & $-$0.068 &  & 0.112 &  \\ 
  & (0.097) &  & (0.103) &  \\ 
  lag(closed movie theaters, 21) &  & 0.006 &  & 0.062 \\ 
  &  & (0.113) &  & (0.101) \\ 
  lag(closed restaurants, 21) &  & $-$0.143 &  & $-$0.043 \\ 
  &  & (0.098) &  & (0.080) \\ 
  lag(closed non-essent bus, 21) &  & 0.074 &  & 0.096 \\ 
  &  & (0.084) &  & (0.085) \\ 
  lag($\Delta \log \Delta D_{it}$, 21) & $-$0.002 & 0.005 & 0.019 & 0.022 \\ 
  & (0.032) & (0.032) & (0.036) & (0.035) \\ 
  lag($\log \Delta D_{it}$, 21) & $-$0.093$^{***}$ & $-$0.099$^{***}$ & $-$0.066$^{**}$ & $-$0.069$^{**}$ \\ 
  & (0.025) & (0.025) & (0.027) & (0.028) \\ 
  lag($\Delta \log \Delta D_{it}$.national, 21) &  &  & $-$0.145$^{***}$ & $-$0.135$^{**}$ \\ 
  &  &  & (0.054) & (0.057) \\ 
  lag($\log \Delta D_{it}$.national, 21) &  &  & $-$0.131$^{***}$ & $-$0.131$^{***}$ \\ 
  &  &  & (0.032) & (0.031) \\ 
   &  &  &  &  \\ 
  &  &  &  &  \\ 
 \hline \\[-1.8ex] 
state variables & Yes & Yes & Yes & Yes \\ 
Month $\times$ state variables & Yes & Yes & Yes & Yes \\ 
\hline \\[-1.8ex] 
$\sum_j \mathrm{Policy}_j$ & -0.771$^{***}$ & -0.716$^{***}$ & -0.326 & -0.295 \\ 
 & (0.185) & (0.202) & (0.210) & (0.218) \\ 
Observations & 3,468 & 3,468 & 3,468 & 3,468 \\ 
R$^{2}$ & 0.496 & 0.498 & 0.512 & 0.512 \\ 
Adjusted R$^{2}$ & 0.491 & 0.492 & 0.506 & 0.507 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables_and_figures/newcasecor.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:36:02 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:40 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & NYT & JHU & CTP \\ 
  \hline
NYT & 1.00 & 0.93 & 0.86 \\ 
  JHU & 0.93 & 1.00 & 0.82 \\ 
  CTP & 0.86 & 0.82 & 1.00 \\ 
  Variance & 5.05 & 5.81 & 6.11 \\ 
   \hline
\end{tabular}
\caption{Correlation and variance of log daily new cases\label{tab:newcasecor}} 
\end{table}


==> tables_and_figures/policies.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:36:07 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:47 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rllll}
  \hline
 & N & Min & Median & Max \\ 
  \hline
State of emergency & 51 & 2020-02-29 & 2020-03-11 & 2020-03-16 \\ 
  Date closed K 12 schools & 51 & 2020-03-13 & 2020-03-17 & 2020-04-03 \\ 
  Closed day cares & 15 & 2020-03-16 & 2020-03-23 & 2020-04-06 \\ 
  Date banned visitors to nursing homes & 30 & 2020-03-09 & 2020-03-16 & 2020-04-06 \\ 
  Closed non essential businesses & 43 & 2020-03-19 & 2020-03-25 & 2020-04-06 \\ 
  Closed restaurants except take out & 48 & 2020-03-15 & 2020-03-17 & 2020-04-03 \\ 
  Closed gyms & 49 & 2020-03-16 & 2020-03-20 & 2020-04-03 \\ 
  Closed movie theaters & 49 & 2020-03-16 & 2020-03-21 & 2020-04-06 \\ 
  Stay at home  shelter in place & 42 & 2020-03-19 & 2020-03-28 & 2020-04-07 \\ 
  End relax stay at home shelter in place & 39 & 2020-04-24 & 2020-05-18 & 2020-06-19 \\ 
  Began to reopen businesses statewide & 50 & 2020-04-20 & 2020-05-07 & 2020-06-05 \\ 
  Reopen restaurants & 48 & 2020-04-24 & 2020-05-18 & 2020-06-22 \\ 
  Reopened gyms & 44 & 2020-04-24 & 2020-05-18 & 2020-07-13 \\ 
  Reopened movie theaters & 37 & 2020-04-27 & 2020-06-01 & 2020-07-13 \\ 
  Resumed elective medical procedures & 35 & 2020-04-20 & 2020-04-30 & 2020-05-29 \\ 
  Mandate face mask use by all individuals in public spaces & 35 & 2020-04-08 & 2020-06-26 & 2020-08-05 \\ 
  Mandate face mask use by employees in public facing businesses & 44 & 2020-04-03 & 2020-05-01 & 2020-08-03 \\ 
  Stop Initiation of Evictions overall or due to COVID related issues & 30 & 2020-03-16 & 2020-03-24 & 2020-05-30 \\ 
  Stop enforcement of evictions overall or due to COVID related issues & 29 & 2020-03-15 & 2020-03-24 & 2020-06-08 \\ 
  Renter grace period or use of security deposit to pay rent & 3 & 2020-04-10 & 2020-04-24 & 2020-05-20 \\ 
  Order freezing utility shut offs & 34 & 2020-03-12 & 2020-03-19 & 2020-04-13 \\ 
  Froze mortgage payments & 1 & 2020-03-21 & 2020-03-21 & 2020-03-21 \\ 
  Waived one week waiting period for unemployment insurance & 36 & 2020-03-08 & 2020-03-18 & 2020-04-06 \\ 
   \hline
\end{tabular}
\caption{State Policies \label{tab:policies}} 
\end{table}


==> tables_and_figures/policies_inregs.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:36:07 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:47 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rllll}
  \hline
 & N & Min & Median & Max \\ 
  \hline
Date closed K 12 schools & 51 & 2020-03-13 & 2020-03-17 & 2020-04-03 \\ 
  Stay at home  shelter in place & 42 & 2020-03-19 & 2020-03-28 & 2020-04-07 \\ 
  Closed movie theaters & 49 & 2020-03-16 & 2020-03-21 & 2020-04-06 \\ 
  Closed restaurants except take out & 48 & 2020-03-15 & 2020-03-17 & 2020-04-03 \\ 
  Closed non essential businesses & 43 & 2020-03-19 & 2020-03-25 & 2020-04-06 \\ 
  Mandate face mask use by employees & 44 & 2020-04-03 & 2020-05-01 & 2020-08-03 \\ 
   \hline
\end{tabular}
\caption{State Policies \label{tab:policies_inreg}} 
\end{table}


==> tables_and_figures/weekcasecor.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:36:02 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:40 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & NYT & JHU & CTP \\ 
  \hline
NYT & 1.00 & 1.00 & 0.98 \\ 
  JHU & 1.00 & 1.00 & 0.98 \\ 
  CTP & 0.98 & 0.98 & 1.00 \\ 
  Variance & 3.68 & 3.76 & 3.47 \\ 
   \hline
\end{tabular}
\caption{Correlation and variance of log weekly new cases\label{tab:weekcasecor}} 
\end{table}


==> tables_and_figures/weekdeathcor.tex <==
<<<<<<< HEAD
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Mon Sep 20 14:36:03 2021
=======
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Tue Aug 24 12:42:41 2021
>>>>>>> parent of c8dc981 (cases_and_policies_update revised)
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & NYT & JHU & CTP \\ 
  \hline
NYT & 1.00 & 0.98 & 0.97 \\ 
  JHU & 0.98 & 1.00 & 0.98 \\ 
  CTP & 0.97 & 0.98 & 1.00 \\ 
  Variance & 172292.15 & 174310.07 & 126952.94 \\ 
   \hline
\end{tabular}
\caption{Correlation and variance of weekly deaths\label{tab:weekdeathcor}} 
\end{table}

